Suppression of Upsilon Production in d+Au and Au+Au Collisions at sqrt(s_NN) = 200 GeV

We report measurements of Upsilon meson production in p+p, d+Au, and Au+Au collisions using the STAR detector at RHIC. We compare the Upsilon yield to the measured cross section in p+p collisions in order to quantify any modifications of the yield in cold nuclear matter using d+Au data and in hot nuclear matter using Au+Au data separated into three centrality classes. Our p+p measurement is based on three times the statistics of our previous result. We obtain a nuclear modification factor for Upsilon(1S+2S+3S) in the rapidity range |y|<1 in d+Au collisions of R_dAu = 0.79 +/- 0.24 (stat.) +/- 0.03 (sys.) +/- 0.10 (pp sys.). A comparison with models including shadowing and initial state parton energy loss indicates the presence of additional cold-nuclear matter suppression. Similarly, in the top 10% most-central Au+Au collisions, we measure a nuclear modification factor of R_AA=0.49 +/- 0.1 (stat.) +/- 0.02 (sys.) +/- 0.06 (pp sys.), which is a larger suppression factor than that seen in cold nuclear matter. Our results are consistent with complete suppression of excited-state Upsilon mesons in Au+Au collisions. The additional suppression in Au+Au is consistent with the level expected in model calculations that include the presence of a hot, deconfined Quark-Gluon Plasma. However, understanding the suppression seen in d+Au is still needed before any definitive statements about the nature of the suppression in Au+Au can be made.

==> AuthorsRevTex.tex <==
\affiliation{AGH University of Science and Technology, Cracow, Poland}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\affiliation{University of Birmingham, Birmingham, United Kingdom}
\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\affiliation{University of California, Berkeley, California 94720, USA}
\affiliation{University of California, Davis, California 95616, USA}
\affiliation{University of California, Los Angeles, California 90095, USA}
\affiliation{Universidade Estadual de Campinas, Sao Paulo, Brazil}
\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\affiliation{Cracow University of Technology, Cracow, Poland}
\affiliation{Creighton University, Omaha, Nebraska 68178, USA}
\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\affiliation{Nuclear Physics Institute AS CR, 250 68 \v{R}e\v{z}/Prague, Czech Republic}
\affiliation{Frankfurt Institute for Advanced Studies FIAS, Germany}
\affiliation{Institute of Physics, Bhubaneswar 751005, India}
\affiliation{Indian Institute of Technology, Mumbai, India}
\affiliation{Indiana University, Bloomington, Indiana 47408, USA}
\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow, Russia}
\affiliation{University of Jammu, Jammu 180001, India}
\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\affiliation{Kent State University, Kent, Ohio 44242, USA}
\affiliation{University of Kentucky, Lexington, Kentucky, 40506-0055, USA}
\affiliation{Korea Institute of Science and Technology Information, Daejeon, Korea}
\affiliation{Institute of Modern Physics, Lanzhou, China}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}
\affiliation{Max-Planck-Institut f\"ur Physik, Munich, Germany}
\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\affiliation{Moscow Engineering Physics Institute, Moscow Russia}
\affiliation{National Institute of Science Education and Research, Bhubaneswar 751005, India}
\affiliation{Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{Old Dominion University, Norfolk, VA, 23529, USA}
\affiliation{Institute of Nuclear Physics PAN, Cracow, Poland}
\affiliation{Panjab University, Chandigarh 160014, India}
\affiliation{Pennsylvania State University, University Park, Pennsylvania 16802, USA}
\affiliation{Institute of High Energy Physics, Protvino, Russia}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\affiliation{Pusan National University, Pusan, Republic of Korea}
\affiliation{University of Rajasthan, Jaipur 302004, India}
\affiliation{Rice University, Houston, Texas 77251, USA}
\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil}
\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\affiliation{Shandong University, Jinan, Shandong 250100, China}
\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\affiliation{SUBATECH, Nantes, France}
\affiliation{Temple University, Philadelphia, Pennsylvania, 19122, USA}
\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\affiliation{University of Texas, Austin, Texas 78712, USA}
\affiliation{University of Houston, Houston, TX, 77204, USA}
\affiliation{Tsinghua University, Beijing 100084, China}
\affiliation{United States Naval Academy, Annapolis, MD 21402, USA}
\affiliation{Valparaiso University, Valparaiso, Indiana 46383, USA}
\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\affiliation{Warsaw University of Technology, Warsaw, Poland}
\affiliation{University of Washington, Seattle, Washington 98195, USA}
\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\affiliation{University of Zagreb, Zagreb, HR-10002, Croatia}

\author{L.~Adamczyk}\affiliation{AGH University of Science and Technology, Cracow, Poland}
\author{J.~K.~Adkins}\affiliation{University of Kentucky, Lexington, Kentucky, 40506-0055, USA}
\author{G.~Agakishiev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{M.~M.~Aggarwal}\affiliation{Panjab University, Chandigarh 160014, India}
\author{Z.~Ahammed}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{I.~Alekseev}\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow, Russia}
\author{J.~Alford}\affiliation{Kent State University, Kent, Ohio 44242, USA}
\author{C.~D.~Anson}\affiliation{Ohio State University, Columbus, Ohio 43210, USA}
\author{A.~Aparin}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{D.~Arkhipkin}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{E.~C.~Aschenauer}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{G.~S.~Averichev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~Balewski}\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}
\author{A.~Banerjee}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{Z.~Barnovska~}\affiliation{Nuclear Physics Institute AS CR, 250 68 \v{R}e\v{z}/Prague, Czech Republic}
\author{D.~R.~Beavis}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{R.~Bellwied}\affiliation{University of Houston, Houston, TX, 77204, USA}
\author{A.~Bhasin}\affiliation{University of Jammu, Jammu 180001, India}
\author{A.~K.~Bhati}\affiliation{Panjab University, Chandigarh 160014, India}
\author{P.~Bhattarai}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{H.~Bichsel}\affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{J.~Bielcik}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{J.~Bielcikova}\affiliation{Nuclear Physics Institute AS CR, 250 68 \v{R}e\v{z}/Prague, Czech Republic}
\author{L.~C.~Bland}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{I.~G.~Bordyuzhin}\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow, Russia}
\author{W.~Borowski}\affiliation{SUBATECH, Nantes, France}
\author{J.~Bouchet}\affiliation{Kent State University, Kent, Ohio 44242, USA}
\author{A.~V.~Brandin}\affiliation{Moscow Engineering Physics Institute, Moscow Russia}
\author{S.~G.~Brovko}\affiliation{University of California, Davis, California 95616, USA}
\author{S.~B{\"u}ltmann}\affiliation{Old Dominion University, Norfolk, VA, 23529, USA}
\author{I.~Bunzarov}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{T.~P.~Burton}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{J.~Butterworth}\affiliation{Rice University, Houston, Texas 77251, USA}
\author{H.~Caines}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{M.~Calder\'on~de~la~Barca~S\'anchez}\affiliation{University of California, Davis, California 95616, USA}
\author{D.~Cebra}\affiliation{University of California, Davis, California 95616, USA}
\author{R.~Cendejas}\affiliation{Pennsylvania State University, University Park, Pennsylvania 16802, USA}
\author{M.~C.~Cervantes}\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\author{P.~Chaloupka}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{Z.~Chang}\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\author{S.~Chattopadhyay}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{H.~F.~Chen}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{J.~H.~Chen}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{L.~Chen}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{J.~Cheng}\affiliation{Tsinghua University, Beijing 100084, China}
\author{M.~Cherney}\affiliation{Creighton University, Omaha, Nebraska 68178, USA}
\author{A.~Chikanian}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{W.~Christie}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{J.~Chwastowski}\affiliation{Cracow University of Technology, Cracow, Poland}
\author{M.~J.~M.~Codrington}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{R.~Corliss}\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}
\author{J.~G.~Cramer}\affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{H.~J.~Crawford}\affiliation{University of California, Berkeley, California 94720, USA}
\author{X.~Cui}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{S.~Das}\affiliation{Institute of Physics, Bhubaneswar 751005, India}
\author{A.~Davila~Leyva}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{L.~C.~De~Silva}\affiliation{University of Houston, Houston, TX, 77204, USA}
\author{R.~R.~Debbe}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{T.~G.~Dedovich}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~Deng}\affiliation{Shandong University, Jinan, Shandong 250100, China}
\author{A.~A.~Derevschikov}\affiliation{Institute of High Energy Physics, Protvino, Russia}
\author{R.~Derradi~de~Souza}\affiliation{Universidade Estadual de Campinas, Sao Paulo, Brazil}
\author{S.~Dhamija}\affiliation{Indiana University, Bloomington, Indiana 47408, USA}
\author{B.~di~Ruzza}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{L.~Didenko}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{C.~Dilks}\affiliation{Pennsylvania State University, University Park, Pennsylvania 16802, USA}
\author{F.~Ding}\affiliation{University of California, Davis, California 95616, USA}
\author{P.~Djawotho}\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\author{X.~Dong}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{J.~L.~Drachenberg}\affiliation{Valparaiso University, Valparaiso, Indiana 46383, USA}
\author{J.~E.~Draper}\affiliation{University of California, Davis, California 95616, USA}
\author{C.~M.~Du}\affiliation{Institute of Modern Physics, Lanzhou, China}
\author{L.~E.~Dunkelberger}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{J.~C.~Dunlop}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{L.~G.~Efimov}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~Engelage}\affiliation{University of California, Berkeley, California 94720, USA}
\author{K.~S.~Engle}\affiliation{United States Naval Academy, Annapolis, MD 21402, USA}
\author{G.~Eppley}\affiliation{Rice University, Houston, Texas 77251, USA}
\author{L.~Eun}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{O.~Evdokimov}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{R.~Fatemi}\affiliation{University of Kentucky, Lexington, Kentucky, 40506-0055, USA}
\author{S.~Fazio}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{J.~Fedorisin}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{P.~Filip}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{E.~Finch}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{Y.~Fisyak}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{C.~E.~Flores}\affiliation{University of California, Davis, California 95616, USA}
\author{C.~A.~Gagliardi}\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\author{D.~R.~Gangadharan}\affiliation{Ohio State University, Columbus, Ohio 43210, USA}
\author{D.~ Garand}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{F.~Geurts}\affiliation{Rice University, Houston, Texas 77251, USA}
\author{A.~Gibson}\affiliation{Valparaiso University, Valparaiso, Indiana 46383, USA}
\author{M.~Girard}\affiliation{Warsaw University of Technology, Warsaw, Poland}
\author{S.~Gliske}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\author{D.~Grosnick}\affiliation{Valparaiso University, Valparaiso, Indiana 46383, USA}
\author{Y.~Guo}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{A.~Gupta}\affiliation{University of Jammu, Jammu 180001, India}
\author{S.~Gupta}\affiliation{University of Jammu, Jammu 180001, India}
\author{W.~Guryn}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{B.~Haag}\affiliation{University of California, Davis, California 95616, USA}
\author{O.~Hajkova}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{A.~Hamed}\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\author{L-X.~Han}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{R.~Haque}\affiliation{National Institute of Science Education and Research, Bhubaneswar 751005, India}
\author{J.~W.~Harris}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{J.~P.~Hays-Wehle}\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}
\author{S.~Heppelmann}\affiliation{Pennsylvania State University, University Park, Pennsylvania 16802, USA}
\author{K.~Hill}\affiliation{University of California, Davis, California 95616, USA}
\author{A.~Hirsch}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{G.~W.~Hoffmann}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{D.~J.~Hofman}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{S.~Horvat}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{B.~Huang}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{H.~Z.~Huang}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{P.~Huck}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{T.~J.~Humanic}\affiliation{Ohio State University, Columbus, Ohio 43210, USA}
\author{G.~Igo}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{W.~W.~Jacobs}\affiliation{Indiana University, Bloomington, Indiana 47408, USA}
\author{H.~Jang}\affiliation{Korea Institute of Science and Technology Information, Daejeon, Korea}
\author{E.~G.~Judd}\affiliation{University of California, Berkeley, California 94720, USA}
\author{S.~Kabana}\affiliation{SUBATECH, Nantes, France}
\author{D.~Kalinkin}\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow, Russia}
\author{K.~Kang}\affiliation{Tsinghua University, Beijing 100084, China}
\author{K.~Kauder}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{H.~W.~Ke}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{D.~Keane}\affiliation{Kent State University, Kent, Ohio 44242, USA}
\author{A.~Kechechyan}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{A.~Kesich}\affiliation{University of California, Davis, California 95616, USA}
\author{Z.~H.~Khan}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{D.~P.~Kikola}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{I.~Kisel}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Germany}
\author{A.~Kisiel}\affiliation{Warsaw University of Technology, Warsaw, Poland}
\author{D.~D.~Koetke}\affiliation{Valparaiso University, Valparaiso, Indiana 46383, USA}
\author{T.~Kollegger}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Germany}
\author{J.~Konzer}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{I.~Koralt}\affiliation{Old Dominion University, Norfolk, VA, 23529, USA}
\author{W.~Korsch}\affiliation{University of Kentucky, Lexington, Kentucky, 40506-0055, USA}
\author{L.~Kotchenda}\affiliation{Moscow Engineering Physics Institute, Moscow Russia}
\author{P.~Kravtsov}\affiliation{Moscow Engineering Physics Institute, Moscow Russia}
\author{K.~Krueger}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\author{I.~Kulakov}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Germany}
\author{L.~Kumar}\affiliation{National Institute of Science Education and Research, Bhubaneswar 751005, India}
\author{R.~A.~Kycia}\affiliation{Cracow University of Technology, Cracow, Poland}
\author{M.~A.~C.~Lamont}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{J.~M.~Landgraf}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{K.~D.~ Landry}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{J.~Lauret}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{A.~Lebedev}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{R.~Lednicky}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~H.~Lee}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{W.~Leight}\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}
\author{M.~J.~LeVine}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{C.~Li}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{W.~Li}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{X.~Li}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{X.~Li}\affiliation{Temple University, Philadelphia, Pennsylvania, 19122, USA}
\author{Y.~Li}\affiliation{Tsinghua University, Beijing 100084, China}
\author{Z.~M.~Li}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{L.~M.~Lima}\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil}
\author{M.~A.~Lisa}\affiliation{Ohio State University, Columbus, Ohio 43210, USA}
\author{F.~Liu}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{T.~Ljubicic}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{W.~J.~Llope}\affiliation{Rice University, Houston, Texas 77251, USA}
\author{R.~S.~Longacre}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{X.~Luo}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{G.~L.~Ma}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{Y.~G.~Ma}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{D.~M.~M.~D.~Madagodagettige~Don}\affiliation{Creighton University, Omaha, Nebraska 68178, USA}
\author{D.~P.~Mahapatra}\affiliation{Institute of Physics, Bhubaneswar 751005, India}
\author{R.~Majka}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{S.~Margetis}\affiliation{Kent State University, Kent, Ohio 44242, USA}
\author{C.~Markert}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{H.~Masui}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{H.~S.~Matis}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{D.~McDonald}\affiliation{Rice University, Houston, Texas 77251, USA}
\author{T.~S.~McShane}\affiliation{Creighton University, Omaha, Nebraska 68178, USA}
\author{N.~G.~Minaev}\affiliation{Institute of High Energy Physics, Protvino, Russia}
\author{S.~Mioduszewski}\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\author{B.~Mohanty}\affiliation{National Institute of Science Education and Research, Bhubaneswar 751005, India}
\author{M.~M.~Mondal}\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\author{D.~A.~Morozov}\affiliation{Institute of High Energy Physics, Protvino, Russia}
\author{M.~G.~Munhoz}\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil}
\author{M.~K.~Mustafa}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{B.~K.~Nandi}\affiliation{Indian Institute of Technology, Mumbai, India}
\author{Md.~Nasim}\affiliation{National Institute of Science Education and Research, Bhubaneswar 751005, India}
\author{T.~K.~Nayak}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{J.~M.~Nelson}\affiliation{University of Birmingham, Birmingham, United Kingdom}
\author{L.~V.~Nogach}\affiliation{Institute of High Energy Physics, Protvino, Russia}
\author{S.~Y.~Noh}\affiliation{Korea Institute of Science and Technology Information, Daejeon, Korea}
\author{J.~Novak}\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{S.~B.~Nurushev}\affiliation{Institute of High Energy Physics, Protvino, Russia}
\author{G.~Odyniec}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{A.~Ogawa}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{K.~Oh}\affiliation{Pusan National University, Pusan, Republic of Korea}
\author{A.~Ohlson}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{V.~Okorokov}\affiliation{Moscow Engineering Physics Institute, Moscow Russia}
\author{E.~W.~Oldag}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{R.~A.~N.~Oliveira}\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil}
\author{M.~Pachr}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{B.~S.~Page}\affiliation{Indiana University, Bloomington, Indiana 47408, USA}
\author{S.~K.~Pal}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{Y.~X.~Pan}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{Y.~Pandit}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{Y.~Panebratsev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{T.~Pawlak}\affiliation{Warsaw University of Technology, Warsaw, Poland}
\author{B.~Pawlik}\affiliation{Institute of Nuclear Physics PAN, Cracow, Poland}
\author{H.~Pei}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{C.~Perkins}\affiliation{University of California, Berkeley, California 94720, USA}
\author{W.~Peryt}\affiliation{Warsaw University of Technology, Warsaw, Poland}
\author{A.~Peterson}\affiliation{University of California, Davis, California 95616, USA}
\author{P.~ Pile}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{M.~Planinic}\affiliation{University of Zagreb, Zagreb, HR-10002, Croatia}
\author{J.~Pluta}\affiliation{Warsaw University of Technology, Warsaw, Poland}
\author{D.~Plyku}\affiliation{Old Dominion University, Norfolk, VA, 23529, USA}
\author{N.~Poljak}\affiliation{University of Zagreb, Zagreb, HR-10002, Croatia}
\author{J.~Porter}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{A.~M.~Poskanzer}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{N.~K.~Pruthi}\affiliation{Panjab University, Chandigarh 160014, India}
\author{M.~Przybycien}\affiliation{AGH University of Science and Technology, Cracow, Poland}
\author{P.~R.~Pujahari}\affiliation{Indian Institute of Technology, Mumbai, India}
\author{H.~Qiu}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{A.~Quintero}\affiliation{Kent State University, Kent, Ohio 44242, USA}
\author{S.~Ramachandran}\affiliation{University of Kentucky, Lexington, Kentucky, 40506-0055, USA}
\author{R.~Raniwala}\affiliation{University of Rajasthan, Jaipur 302004, India}
\author{S.~Raniwala}\affiliation{University of Rajasthan, Jaipur 302004, India}
\author{R.~L.~Ray}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{C.~K.~Riley}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{H.~G.~Ritter}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{J.~B.~Roberts}\affiliation{Rice University, Houston, Texas 77251, USA}
\author{O.~V.~Rogachevskiy}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~L.~Romero}\affiliation{University of California, Davis, California 95616, USA}
\author{J.~F.~Ross}\affiliation{Creighton University, Omaha, Nebraska 68178, USA}
\author{A.~Roy}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{L.~Ruan}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{J.~Rusnak}\affiliation{Nuclear Physics Institute AS CR, 250 68 \v{R}e\v{z}/Prague, Czech Republic}
\author{N.~R.~Sahoo}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{P.~K.~Sahu}\affiliation{Institute of Physics, Bhubaneswar 751005, India}
\author{I.~Sakrejda}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{S.~Salur}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{A.~Sandacz}\affiliation{Warsaw University of Technology, Warsaw, Poland}
\author{J.~Sandweiss}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{E.~Sangaline}\affiliation{University of California, Davis, California 95616, USA}
\author{A.~ Sarkar}\affiliation{Indian Institute of Technology, Mumbai, India}
\author{J.~Schambach}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{R.~P.~Scharenberg}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{A.~M.~Schmah}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{W.~B.~Schmidke}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{N.~Schmitz}\affiliation{Max-Planck-Institut f\"ur Physik, Munich, Germany}
\author{J.~Seger}\affiliation{Creighton University, Omaha, Nebraska 68178, USA}
\author{P.~Seyboth}\affiliation{Max-Planck-Institut f\"ur Physik, Munich, Germany}
\author{N.~Shah}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{E.~Shahaliev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{P.~V.~Shanmuganathan}\affiliation{Kent State University, Kent, Ohio 44242, USA}
\author{M.~Shao}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{B.~Sharma}\affiliation{Panjab University, Chandigarh 160014, India}
\author{W.~Q.~Shen}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{S.~S.~Shi}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{Q.~Y.~Shou}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{E.~P.~Sichtermann}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{R.~N.~Singaraju}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{M.~J.~Skoby}\affiliation{Indiana University, Bloomington, Indiana 47408, USA}
\author{D.~Smirnov}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{N.~Smirnov}\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{D.~Solanki}\affiliation{University of Rajasthan, Jaipur 302004, India}
\author{P.~Sorensen}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{U.~G.~deSouza}\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil}
\author{H.~M.~Spinka}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\author{B.~Srivastava}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{T.~D.~S.~Stanislaus}\affiliation{Valparaiso University, Valparaiso, Indiana 46383, USA}
\author{J.~R.~Stevens}\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}
\author{R.~Stock}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Germany}
\author{M.~Strikhanov}\affiliation{Moscow Engineering Physics Institute, Moscow Russia}
\author{B.~Stringfellow}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{A.~A.~P.~Suaide}\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil}
\author{M.~Sumbera}\affiliation{Nuclear Physics Institute AS CR, 250 68 \v{R}e\v{z}/Prague, Czech Republic}
\author{X.~Sun}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{X.~M.~Sun}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{Y.~Sun}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{Z.~Sun}\affiliation{Institute of Modern Physics, Lanzhou, China}
\author{B.~Surrow}\affiliation{Temple University, Philadelphia, Pennsylvania, 19122, USA}
\author{D.~N.~Svirida}\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow, Russia}
\author{T.~J.~M.~Symons}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{A.~Szanto~de~Toledo}\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil}
\author{J.~Takahashi}\affiliation{Universidade Estadual de Campinas, Sao Paulo, Brazil}
\author{A.~H.~Tang}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{Z.~Tang}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{T.~Tarnowsky}\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{J.~H.~Thomas}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{A.~R.~Timmins}\affiliation{University of Houston, Houston, TX, 77204, USA}
\author{D.~Tlusty}\affiliation{Nuclear Physics Institute AS CR, 250 68 \v{R}e\v{z}/Prague, Czech Republic}
\author{M.~Tokarev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{S.~Trentalange}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{R.~E.~Tribble}\affiliation{Texas A\&M University, College Station, Texas 77843, USA}
\author{P.~Tribedy}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{B.~A.~Trzeciak}\affiliation{Warsaw University of Technology, Warsaw, Poland}
\author{O.~D.~Tsai}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{J.~Turnau}\affiliation{Institute of Nuclear Physics PAN, Cracow, Poland}
\author{T.~Ullrich}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{D.~G.~Underwood}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\author{G.~Van~Buren}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{G.~van~Nieuwenhuizen}\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}
\author{J.~A.~Vanfossen,~Jr.}\affiliation{Kent State University, Kent, Ohio 44242, USA}
\author{R.~Varma}\affiliation{Indian Institute of Technology, Mumbai, India}
\author{G.~M.~S.~Vasconcelos}\affiliation{Universidade Estadual de Campinas, Sao Paulo, Brazil}
\author{A.~N.~Vasiliev}\affiliation{Institute of High Energy Physics, Protvino, Russia}
\author{R.~Vertesi}\affiliation{Nuclear Physics Institute AS CR, 250 68 \v{R}e\v{z}/Prague, Czech Republic}
\author{F.~Videb{\ae}k}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{Y.~P.~Viyogi}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{S.~Vokal}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{A.~Vossen}\affiliation{Indiana University, Bloomington, Indiana 47408, USA}
\author{M.~Wada}\affiliation{University of Texas, Austin, Texas 78712, USA}
\author{M.~Walker}\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}
\author{F.~Wang}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{G.~Wang}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{H.~Wang}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{J.~S.~Wang}\affiliation{Institute of Modern Physics, Lanzhou, China}
\author{X.~L.~Wang}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{Y.~Wang}\affiliation{Tsinghua University, Beijing 100084, China}
\author{Y.~Wang}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{G.~Webb}\affiliation{University of Kentucky, Lexington, Kentucky, 40506-0055, USA}
\author{J.~C.~Webb}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{G.~D.~Westfall}\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{H.~Wieman}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{G.~Wimsatt}\affiliation{University of California, Davis, California 95616, USA}
\author{S.~W.~Wissink}\affiliation{Indiana University, Bloomington, Indiana 47408, USA}
\author{R.~Witt}\affiliation{United States Naval Academy, Annapolis, MD 21402, USA}
\author{Y.~F.~Wu}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{Z.~Xiao}\affiliation{Tsinghua University, Beijing 100084, China}
\author{W.~Xie}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{K.~Xin}\affiliation{Rice University, Houston, Texas 77251, USA}
\author{H.~Xu}\affiliation{Institute of Modern Physics, Lanzhou, China}
\author{N.~Xu}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{Q.~H.~Xu}\affiliation{Shandong University, Jinan, Shandong 250100, China}
\author{Y.~Xu}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{Z.~Xu}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{W.~Yan}\affiliation{Tsinghua University, Beijing 100084, China}
\author{C.~Yang}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{Y.~Yang}\affiliation{Institute of Modern Physics, Lanzhou, China}
\author{Y.~Yang}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{Z.~Ye}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{P.~Yepes}\affiliation{Rice University, Houston, Texas 77251, USA}
\author{L.~Yi}\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{K.~Yip}\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{I-K.~Yoo}\affiliation{Pusan National University, Pusan, Republic of Korea}
\author{Y.~Zawisza}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{H.~Zbroszczyk}\affiliation{Warsaw University of Technology, Warsaw, Poland}
\author{W.~Zha}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{J.~B.~Zhang}\affiliation{Central China Normal University (HZNU), Wuhan 430079, China}
\author{J.~L.~Zhang}\affiliation{Shandong University, Jinan, Shandong 250100, China}
\author{S.~Zhang}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{X.~P.~Zhang}\affiliation{Tsinghua University, Beijing 100084, China}
\author{Y.~Zhang}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{Z.~P.~Zhang}\affiliation{University of Science \& Technology of China, Hefei 230026, China}
\author{F.~Zhao}\affiliation{University of California, Los Angeles, California 90095, USA}
\author{J.~Zhao}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{C.~Zhong}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{X.~Zhu}\affiliation{Tsinghua University, Beijing 100084, China}
\author{Y.~H.~Zhu}\affiliation{Shanghai Institute of Applied Physics, Shanghai 201800, China}
\author{Y.~Zoulkarneeva}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{M.~Zyzak}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Germany}

\collaboration{STAR Collaboration}\noaffiliation

